A Computationally-Efficient Closed-Form $C^{s,1}$-Extension Formula

We identify explicit closed-form and variational formulae for interpolating the exact values and derivatives through order $s$ of a $C^{s,1}$ function $f:\mathbb{R}^d\to\mathbb{R}$ at $N$ distinct points in $[0,1]^d$. The reconstruction satisfies bounds on its global $C^{s,1}$ seminorm and its Lipschitz constant on $[0,1]^d$ that are independent of the sample size $N$, the latter being the sharp Whitney condition. For $s\ge2$, the reconstruction is real analytic away from the data points and definable in the o-minimal structure $\mathbb{R}_{\exp}$. Our nonlinear extension formula coincides with the formula of McShane (1934) for $s=0$ and with the formulae of Le Gruyer and Phan (2015) and Azagra, Le Gruyer, and Mudarra (2018) for $s=1$, and is new for $s\ge2$. For fixed $d$ and $s\ge2$, our closed-form formula is computable away from the data points by a circuit using only elementary unary and binary real operations, with $\mathcal{O}(N)$ gates and $\mathcal{O}(\log N)$ depth. This yields $\mathcal{O}(N)$ storage and $\mathcal{O}(\log N)$ parallel evaluation time. From the supplied coefficients and weights, the circuit can be compiled with $\mathcal{O}(N)$ one-time work in the exact-real word-RAM model. Thus, in this supplied-data setting, our nonlinear construction improves by a logarithmic factor on the $\mathcal{O}(N\log N)$ initialization bound of Fefferman and Klartag (2009), while retaining linear storage and attaining logarithmic query time through parallel evaluation.

==> Code/Experiments/jet_visualization/whitney_dual-0.1.0.dist-info/METADATA <==
Metadata-Version: 2.4
Name: whitney-dual
Version: 0.1.0
Summary: Differentiable PyTorch evaluation of the entropy-variance Whitney extension dual
Requires-Python: >=3.10
Description-Content-Type: text/markdown
Requires-Dist: torch>=2.2
Provides-Extra: test
Requires-Dist: pytest>=8; extra == "test"
Requires-Dist: numpy>=1.26; extra == "test"
Requires-Dist: scipy>=1.12; extra == "test"

# Whitney dual in PyTorch

Evaluates the **s ≥ 2 entropy–variance Whitney extension** by solving its
equivalent unconstrained dual in **d variables**. It uses every supplied site;
each objective evaluation still depends on N. The package includes batching,
implicit autograd, convergence diagnostics, independent primal tests, and a
reproducible benchmark. **Sparse polynomial inputs stay sparse:** only supplied
monomials are evaluated, without constructing the full degree-s basis.

The source is `Pasted text(20260925-032925).txt`, specifically
`eq:entropy-variance-extension`, `eq:gibbs-dual-quantities`, and
`eq:dualization-direct-gap`. The earlier supplied `032628` copy is byte-identical.
See [the mathematics-to-code contract](docs/MATHEMATICS.md) for derivations and
assumptions, and [the verification report](docs/VERIFICATION.md) for actual runs.

## Install and run

Unzip the source archive, open a terminal in its `whitney-dual` directory, and run:

```bash
python -m pip install .
python examples/sparse_polynomials.py
```

Alternatively, install the supplied wheel directly:

```bash
python -m pip install whitney_dual-0.1.0-py3-none-any.whl
```

A wheel is the installable Python package. The source archive also contains the
tests, explanations, examples, and benchmark. PyTorch is the only runtime
dependency; a compatible installation is needed if installing offline.

## Sparse polynomials: the primary interface

Give each location and its nonzero `(multi-index, coefficient)` pairs:

```python
import torch
from whitney_dual import SparseWhitneyDual

# Local Taylor polynomials for f(x,y)=x²+3y at (0,0) and (1,0).
records = [
    ([0.0, 0.0], {(2, 0): 1.0, (0, 1): 3.0}),
    ([1.0, 0.0], {(0, 0): 1.0, (1, 0): 2.0,
                  (2, 0): 1.0, (0, 1): 3.0}),
]
F = SparseWhitneyDual.from_polynomials(records, order=2, M=1.0)
x = torch.tensor([[0.2, 0.1], [0.8, -0.2]], dtype=torch.float64,
                 requires_grad=True)
values = F(x)
gradient, = torch.autograd.grad(values.sum(), x)
info = F.evaluate(x)
print(values, gradient, info.gap)
```

By default a term means **`coefficient * (x - location)**multi_index`**, with
the product over coordinates understood. Coefficients are polynomial
coefficients, so Taylor data use `D^alpha f(location)/alpha!`.
Set `basis="global"` if terms instead mean `coefficient * x**multi_index`.
An omitted monomial means its coefficient is exactly zero; it does not mean a
missing derivative measurement. Each polynomial can have a different support.
Lists of `(multi_index, coefficient)` pairs are also accepted; repeated terms
are added. The returned `F` is reusable and supports PyTorch autograd.

`F.polynomials(x)` returns the supplied polynomial values and gradients.
Save the reusable extension with `F.save("extension.pt")` and restore it with
`SparseWhitneyDual.load("extension.pt", map_location="cpu")`.

For tensor-based pipelines, construct `SparseWhitneyDual` directly from
`sites[N,d]`, `term_sites[T]`, `multiindices[T,d]`, and `coefficients[T]`.
The integer tensors identify each stored term's site and exponent vector.
`sparse_whitney_dual` is the corresponding functional interface for trainable
inputs. The sparse representation uses T supplied terms; it never allocates
N times `binom(d+s,s)` coefficients. The solver still uses N sites and d dual
variables, so sparsity reduces polynomial storage and evaluation rather than
the dimension of the dual.

## Dense jets and automatic derivative extraction

```python
import torch
from whitney_dual import WhitneyDual, jets_from_function

sites = torch.tensor([[-1.0], [0.0], [1.0]], dtype=torch.float64)
# For f(x)=sin(x), Lip(f'') <= 1 on the whole real line.
coefficients = jets_from_function(lambda z: z[0].sin(), sites, order=2)
model = WhitneyDual(sites, coefficients, order=2, M=1.0)

x = torch.tensor([[-0.7], [0.25], [0.8]], dtype=torch.float64,
                 requires_grad=True)
result = model.evaluate(x)
gradient, = torch.autograd.grad(result.value.sum(), x, create_graph=True)
curvature, = torch.autograd.grad(gradient.sum(), x)
print(result.value, gradient, curvature)
print("primal-dual gap:", result.gap)
```

If derivatives have already been measured, supply their Taylor coefficients
directly. `jets_from_function` is a convenience for a differentiable scalar
PyTorch function; it cannot recover derivatives from function values alone.

## Inputs and outputs

| Input | Shape / convention |
|---|---|
| `sites` | `(N, d)`, finite, distinct rows |
| dense `coefficients` | `(N, K)`, where `K = binom(d+s, s)` |
| dense coefficient column α | `D^α f(X_i) / α!`; order given by `multi_indices(d, s)` |
| `order` | Integer `s >= 2` |
| `M` | Positive scalar or scalar tensor; witness seminorm bound is the caller's responsibility |
| `mu` | Optional positive site weights summing to one; default uniform |
| `q` | Optional positive exponent; default `2*s + 46*d + 2` |
| `x` | `(..., d)`, arbitrary query batch shape |
| dtype / device | All floating tensors must share `float64` or `float32` and a device |

`model(x)` returns values with shape `x.shape[:-1]`.
`model.evaluate(x)` additionally returns `gap`, `weights`, `converged`,
`iterations`, `gradient_norm`, `u`, and `at_sites`. `primal_value` is the
corresponding upper value obtained from the Gibbs weights, computed as
`value + gap`. `u` and `gradient_norm` use normalized dual coordinates; `gap`
uses the original function-value scale. At exact sample sites, diagnostics use
the prescribed polynomial branch and one-hot site weights; no off-site
optimization is performed.

Use **float64** for research calculations. For float32, explicitly request
attainable solver tolerances, for example `atol=1e-6, rtol=1e-5`. The normalized
stationarity criterion is
`gradient_norm <= atol + rtol * max(1, norm(u-u_initial))`, where `u_initial`
is the reference-weighted feature barycenter. These are residual tolerances,
not a requested absolute error in F. Inspect the original-scale `gap`.
`strict=True` raises when a solve fails to meet the requested criterion.
`strict=False` is for inspecting unsuccessful solves, not accepting them as
converged results.

## What is computed

With β = s−1, p = 2s, and A_s = 1/(s+1)! + β/2, the package forms the
manuscript's θ, R, v, a, c, and τ. It centers the polynomial values and gradients
at a nearest site and rescales the dual algebraically. Its internal problem is

\[
\min_{u\in\mathbb R^d} H(u),\qquad
H(u)=\tfrac12\lVert u\rVert^2+
\log\sum_i\exp\{\log\theta_i-\mathrm{cost}_i
 +\tfrac12\lVert w_i\rVert^2-u\cdot w_i\}.
\]

The Hessian is `I + Cov(weights, w)`. Damped Newton iterations use stable
log-sum-exp, and implicit differentiation uses this Hessian. No optimization
trajectory needs to be retained for the backward pass. The exact-real-arithmetic
gap identity is

\[
0\le F(x)-F_{\rm dual}(x)
\le \frac{\tau(x)}2\left\|u-\sum_i\lambda_i(u)w_i\right\|^2.
\]

The reported floating-point gap is a useful numerical diagnostic; it is **not
an interval-arithmetic certificate**, and it excludes rounding in geometry and
jet evaluation. The implicit derivatives approximate those of the converged
mathematical optimum, rather than derivatives of a finite Newton trajectory.

## Autograd and fitted data

`WhitneyDual` stores supplied data as fixed module buffers for inference and
serialization. Use the functional API when learning coefficients, masses,
sites, or M:

```python
from whitney_dual import whitney_dual

trainable_coefficients = torch.nn.Parameter(coefficients.clone())
raw_M = torch.nn.Parameter(torch.tensor(0.5, dtype=torch.float64))
optimizer = torch.optim.Adam([trainable_coefficients, raw_M], lr=1e-3)
optimizer.zero_grad()
fit = whitney_dual(x, sites, trainable_coefficients, order=2,
                  M=torch.nn.functional.softplus(raw_M))
loss = fit.value.square().mean()
loss.backward()
optimizer.step()
```

Positive parameterizations such as softplus for M and softmax for μ are caller
choices. Free training does not preserve the hypothesis that the jets come
from a common witness with seminorm at most M. The code checks algebraic input
validity, not that functional-analytic assumption.

At an exactly equal site, the branch evaluates its Taylor polynomial rather
than just returning a detached scalar. This preserves the supplied query
derivatives through order s. It does not verify the off-site gluing theorem for
arbitrary input jets. No small-radius snapping is used. The nearest-site
reference only changes dual coordinates; it does not discard other sites.

## Scope and limitations

- Implements the positive-M, s ≥ 2 dual. The s = 0, s = 1, and calibrated
  zero-seminorm polynomial branches are not included.
- The default q matches the manuscript's `D = 2^(46d)`. Its geometric theorem
  also assumes μ has that doubling bound. Uniform μ suffices when
  `N <= 2^(46d)` because `D = N` is a valid bound. For general positive μ,
  `1/min(mu)` (after normalization) is a sufficient bound. The package does not
  construct the manuscript's doubling measure or independently establish a
  supplied geometric certificate. A custom q evaluates a different member of
  the algebraic family and carries no automatic canonical theorem claim.
- With M > 0, even common polynomial data generally do **not** reproduce that
  polynomial away from sites. For N = 1, the result is
  `P_1(x) + A_s*M*||x-X_1||^(s+1)`.
- Extreme scales can overflow normalized powers or lose significant digits.
  Nonfinite computations raise errors. There is no claim of uniform
  floating-point accuracy over all admissible finite geometries.
- With T stored terms, sparse polynomial values/gradients take
  `O(B*T*d*max(1,log(s+1)))` operations using multiplication-based powers,
  with no full monomial enumeration. Sparse metadata uses `O(T*d)` storage.
- Newton uses dense d-by-d linear algebra. Each iteration costs
  `O(B*N*d^2 + B*d^3)`, plus `O(B*N*d)` per line-search evaluation. Geometry and
  polynomial work also depend on the intrinsic jet size `K = binom(d+s,s)`.
  Query batches can be split by the caller to limit memory.
- Tensor calculations stay on the input device. Python convergence/validation
  decisions can synchronize accelerators. GPU execution depends on the device
  supporting the required dtype and linear algebra; consult the verification
  report for devices actually tested. `torch.compile`, `torch.func` transforms,
  forward-mode AD, and mixed precision are not supported contracts.

## Reproduce the checks

```bash
python -m pip install '.[test]'
python -m pytest -q
python benchmarks/benchmark.py --output benchmark_results.json
```

The implementation does not sample during evaluation and is deterministic on
the tested CPU. Sparse index accumulation can be nondeterministic on
accelerators. Examples, independent randomized tests, and benchmarks use documented seeds.
See [docs/VERIFICATION.md](docs/VERIFICATION.md) for the mathematical,
adversarial, and software reviews, numerical comparisons, and measured timings.

